A network-ready random-access qubits memory

Photonic qubits memories are essential ingredients of numerous quantum networking protocols. The ideal situation features quantum computing nodes that are efficiently connected to quantum communication channels via quantum interfaces. The nodes contain a set of long-lived matter qubits, the channels support the propagation of light qubits, and the interface couples light and matter qubits. Towards this vision, we here demonstrate a random-access multi-qubit write-read memory for photons using two rubidium atoms coupled to the same mode of an optical cavity, a setup which is known to feature quantum computing capabilities. We test the memory with more than ten independent photonic qubits, observe no noticeable cross talk, and find no need for re-initialization even after ten write-read attempts. The combined write-read efficiency is 26% and the coherence time approaches 1ms. With these features, the node constitutes a promising building block for a quantum repeater and ultimately a quantum internet.

==> TwoAtomCavityDiagramSymmetric.tex <==
\usetikzlibrary{arrows.meta}
\def\masterfile {}
% colors used for the Rabi driving an the cavity coupling
\definecolor{cR1} {HTML}{009955}
\definecolor{cR2} {HTML}{0000FF}
\definecolor{cR3} {HTML}{0000FF}
\definecolor{cC1} {HTML}{FF0000}
\definecolor{cC2} {HTML}{AA0000}
% more colors
\definecolor{AtomicDecayColor} {HTML}{AA0000}
\input{general.tikz}
\input{arrows.tikz}
\input{cavity.tikz}
\pgfdeclarelayer{bg} % declare background layer
\pgfsetlayers{main,bg} % set the order of the layers (main is the standard layer)

\def\FiveLevelStirapVar(#1){
		% Dimensional definitions
		\renewcommand\zeemansplitting{0.0}
		\renewcommand\mfspacing{1}
		\renewcommand\Fspacing{0.6}
		\renewcommand\GExtSpacing{6.5}
		\renewcommand\lvlwidth{0.7}
		\renewcommand\descriptionspacing{10.5}
		\def\splittingarrowoffset {2.5}

		% the next two function generate coordinates named like F-1-mf--1
		\genGroundStateCoordinates
		\genExtCoordinates(3) % the parameter defines the max F'
		\ifnum #1=2
		\begin{scope}[font=\footnotesize, shift={(7,0)}]
			%\DrawExtCoordinateDesc(1) % add the F' labels
			\node at (-\descriptionspacing*\mfspacing,{\GExtSpacing+\Fspacing}) {$F'=1$};
			\node at (-\descriptionspacing*\mfspacing,{\GExtSpacing+0}) {$F'=0$};
		% and the descriptions for F anf mf
			\node at (-\descriptionspacing*\mfspacing,0.1) {$m_F=$};
			\node at (-\descriptionspacing*\mfspacing,{1.5*1*\Fspacing}) {$F=1$};
			\node at (-\descriptionspacing*\mfspacing,{1.5*2*\Fspacing}) {$F=2$};
		\end{scope}
		\fi
		% an additional coordinate for the detuning level
		\coordinate (detlevel) at ($(Fp-1-mf-1)-(0,1)$);
		\coordinate (detlevel2) at ($(Fp-1-mf--1)-(0,1)$);
		\ifnum #1=2
			\node at ($(Fp-1-mf-0)+(0.0,1)$) {atom A};
		\else
			\node at ($(Fp-1-mf-0)+(0.0,1)$) {atom B};
		\fi
		% draw the levels 
		%\draw[dashed, line width=0.4mm, line cap=round] 
		%($(Fp-1-mf--1)-(0.3,1)$) -- ($(Fp-1-mf-1)-(-0.3,1)$);
		\levelDet(detlevel,,,,)
		\levelDet(detlevel2,,,,)
		\level2 (F-1-mf-0, , , )
		\level2 (F-2-mf-1, , , )
		\level2 (F-2-mf--1, , , )
		\levelGray (F-1-mf-1, , , )
		\levelGray (F-1-mf--1, , , )
		\level2 (F-1-mf-0, , , )
		\levelGray (F-2-mf-0, , , )
		\levelGray (F-2-mf-2, , , )
		\levelGray (F-2-mf--2, , , )
		\level2 (Fp-1-mf-1, , , )
		\level2 (Fp-1-mf--1, , , )
		\levelGray (Fp-1-mf-0, , , )
		\levelGray (Fp-0-mf-0, , , )

		% this loop generate the mf labels 
		\foreach \mf in {-2,...,2} {
				\coordinate (label) at ({\mfspacing*\mf},0.2);
				\node [font=\footnotesize]at (label) {$\mf$};
		}
		\draw [<->, line width=0.5] ($(detlevel)+(0.59,0)$) -- ($(Fp-1-mf-1)+(0.59,0)$) node[pos=0.5,right] {$\Delta$}; 

		% driving arrows 
		% parameter 1,2: start/end coordinate
		% parameter 3,4: small offset the move the the center of the coordinate (if multiple arrows arrive at the same lvl)
		% paramter 5: label
		% paramter 6: position node
		% paramter 7: position coefficient
		% paramter 8: color
		
		%\PhotonArrowNg (F-1-mf-0,detlevell, 0.0,0.05,,right ,pos=0.5,cC1 )
		% parameters are basically the same. However, the color comes earlier
		\ifnum #1=2
			\RabiArrow (detlevel,F-2-mf-1, -0.10, , cR2,right, pos=0.50)
			\RabiArrow (detlevel2,F-2-mf--1, +0.10, $\Omega$, cR2,left, pos=0.50)
		\else
			%\DecayArrow (detlevel,F-2-mf-0, 0.0, 0.1, ,right ,pos=0.5,AtomicDecayColor )
			%\DecayArrow (detlevel,F-2-mf-1, 0.0, 0.1, ,right ,pos=0.5,AtomicDecayColor )
			\DecayArrow (detlevel,{$(F-2-mf-1)+(0.4,1)$}, 0.0, 0., ,right ,pos=0.5,AtomicDecayColor )
			\DecayArrow (detlevel2,{$(F-2-mf--1)+(-0.4,1)$}, 0.0, 0., $\gamma$,left ,pos=0.5,AtomicDecayColor )
		\fi
		
		\PhotonArrowNg (F-1-mf-0,detlevel, 0.0,0.05,$g_{\sigma^+}$,right ,pos=0.9,cC1 )
		\PhotonArrowNg (F-1-mf-0,detlevel2, 0.0,-0.05,$g_{\sigma^-}$,right ,pos=0.9,cC1 )
		
		%\begin{pgfonlayer}{main}
		\ifnum #1=2
			\shade[inner color=gray, outer color=black] ($(F-2-mf-1)+(0,0.28)$) circle (0.8em);
			\shade[inner color=gray, outer color=black] ($(F-2-mf--1)+(0,0.28)$) circle (0.8em);
		\else
			\begin{scope}[transparency group, opacity=0.5]	
				\shade[inner color=gray, outer color=black] ($(F-2-mf-0)+(0,0.28)$) circle (0.8em);
				\shade[inner color=gray, outer color=black] ($(F-2-mf-1)+(0,0.28)$) circle (0.8em);
				\shade[inner color=gray, outer color=black] ($(F-2-mf-2)+(0,0.28)$) circle (0.8em);
				\shade[inner color=gray, outer color=black] ($(F-2-mf--1)+(0,0.28)$) circle (0.8em);
				\shade[inner color=gray, outer color=black] ($(F-2-mf--2)+(0,0.28)$) circle (0.8em);
			\end{scope}
		\fi
		%\end{pgfonlayer}
}

\def\DoubleAtomCavityDiagramSymmetric 
{
\genGroundStateCoordinates
\renewcommand\descriptionspacing{4.5}
\renewcommand\Gspacing {1.5}
\genGroundStateCoordinates
\genExtCoordinates(3)
\def\descriptionspacing{2.1}
\def\spacing{0.15}
%%%%%%%%%%%%%%%%%%%
%
% Cavity
%
%%%%%%%%%%%%%%%%%%%
\begin{scope}[yscale=0.8,xscale=0.8]
%\begin{scope}[shift={(-1.0,-0.20)},yscale=0.285,xscale=0.20,rotate=0]
%\coordinate (cavm1) at (0.8,12);
%\coordinate (cavm2) at (0.8,-2);
%\coordinate (cavm3) at (3.2,-2);
%\coordinate (cavm4) at (3.2,12);
%\definecolor{myred}{rgb}{1,0.5,0.5}
%\draw [fill=myred, draw=none] (cavm1) to [bend left=12] (cavm2) -- (cavm3) to [bend left=12] (cavm4);
%\cavityMirrorDown
%	\begin{scope}[yscale=-1, shift={(0,-1+\cavSpacing*2.4)}]
%	\cavityMirrorUp
%	\end{scope}
%\end{scope}
%%%%%%%%%%%%%%%%%%%
%
% Atom 1
%
%%%%%%%%%%%%%%%%%%%
\begin{scope}[xscale=0.7, yscale=0.6,shift={(2.1,-1.5)}]
	\FiveLevelStirapVar(2)
\end{scope}
%%%%%%%%%%%%%%%%%%%
%
% Atom 2
%
%%%%%%%%%%%%%%%%%%%
\begin{scope}[xscale=0.7, yscale=0.6,shift={(7.5,-1.5)}]
	\FiveLevelStirapVar(1)
\end{scope}
\end{scope}
}


